Individual subpulses of PSR B1916+14 and their polarization properties

Individual subpulses of pulsars are regarded as the basic emission components, providing invaluable information to understand the radio emission process in the pulsar magnetosphere. Nevertheless, subpulses are overlapped with each other along the rotation phase for most pulsars, making it difficult to study the statistical properties of subpulses. Among the pulsars observed by the Five-hundred-meter Aperture Spherical radio Telescope, PSR B1916+14 has a large number of isolated well-resolved subpulses in the high time resolution observations, having a typical width of 0.15 ms and a high linear polarization. We find that the number distribution of subpulses contributes dominantly to the mean profile. According to the emission geometry, these emission units come from a region roughly 155 km above the polar cap in the pulsar magnetosphere, and the length scale of basic emission units is approximately 120 m. The deviations of polarization position angles for these single subpulses from the standard S-shaped curve are closely related to their fractional linear and circular polarization, and the large deviations tend to come from drifting subpulses.

==> individual10.tex <==

\clearpage
\begin{figure*}
\centering
% \includegraphics[width=0.95\textwidth]{singlePulses/singlePulses_0001.pdf}
% \includegraphics[width=0.95\textwidth]{singlePulses/singlePulses_0002.pdf}
% \includegraphics[width=0.95\textwidth]{singlePulses/singlePulses_0003.pdf}
% \includegraphics[width=0.95\textwidth]{singlePulses/singlePulses_0004.pdf}
\includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0013.pdf}
\includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0014.pdf}
\includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0015.pdf}
\includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0016.pdf}
\caption{Polarization profiles for individual Pulses with a time resolution of about 49 $\upmu$s from the FAST observation on May 28th, 2020. One panel for a period, with the period number marked in the lower subpanel, where the total power $I$, linear polarization intensity $L$ and circular polarization intensity are shown, and compared with the enlarged version (x12) of the mean polarization profiles plotted in fainter version. The dashed green line indicates the threshold of $20\sigma_{\rm I}$ obtained from off-pulse data. The PA values of this individual pulses are shown in the upper-subpanel for all bins if their PA have an uncertainty $< 5^\circ$. The PA curve of the mean profile plotted in (red) dots, together with the fitted S-shaped curve (in the dashed grey line), are plotted for comparison.}
\label{fig-individual}
\end{figure*} %\addtocounter{figure}{-1}

% \clearpage
% \begin{figure*}
% \centering
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0005.pdf}
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0006.pdf}
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0007.pdf}
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0008.pdf}
% \caption{Continued from previous page.}
% \label{SP1}
% \end{figure*} \addtocounter{figure}{-1}

% \clearpage
% \begin{figure*}
% \centering
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0009.pdf}
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0010.pdf}
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0011.pdf}
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0012.pdf}
% \caption{Continued from previous page.}
% \label{SP2}
% \end{figure*} \addtocounter{figure}{-1}

% \clearpage
% \begin{figure*}
% \centering
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0013.pdf}
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0014.pdf}
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0015.pdf}
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0016.pdf}
% \caption{Continued from previous page.}
% \label{SP3}
% \end{figure*} \addtocounter{figure}{-1}

% \clearpage
% \begin{figure*}
% \centering
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0017.pdf}
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0018.pdf}
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0019.pdf}
% \includegraphics[width=0.99\textwidth]{singlePulses/singlePulses_0020.pdf}
% \caption{Continued from previous page.}
% \label{SP4}
% \end{figure*} \addtocounter{figure}{-1}


